Temporal Dynamics Decoupling with Inverse Processing for Enhancing Human Motion Prediction

Exploring the bridge between historical and future motion behaviors remains a central challenge in human motion prediction. While most existing methods incorporate a reconstruction task as an auxiliary task into the decoder, thereby improving the modeling of spatio-temporal dependencies, they overlook the potential conflicts between reconstruction and prediction tasks. In this paper, we propose a novel approach: Temporal Decoupling Decoding with Inverse Processing (\textbf{$TD^2IP$}). Our method strategically separates reconstruction and prediction decoding processes, employing distinct decoders to decode the shared motion features into historical or future sequences. Additionally, inverse processing reverses motion information in the temporal dimension and reintroduces it into the model, leveraging the bidirectional temporal correlation of human motion behaviors. By alleviating the conflicts between reconstruction and prediction tasks and enhancing the association of historical and future information, \textbf{$TD^2IP$} fosters a deeper understanding of motion patterns. Extensive experiments demonstrate the adaptability of our method within existing methods.

==> README <==

January 11, 2007


IEEEtran.bst is the official BibTeX style for authors of the Institute of
Electrical and Electronics Engineers (IEEE) Transactions journals and
conferences.

It also may have applications for other academic work such as theses and
technical reports. The alphanumeric and natbib variants extend the
applicability of the IEEEtran bibstyle family to the natural sciences
and beyond.

The IEEEtran bibstyle is a very comprehensive BibTeX style which provides
many features beyond the standard BibTeX styles, including full support
for references of online documents, patents, periodicals and standards.
See the provided user manual for detailed usage information.

The latest version of the IEEEtran BibTeX style can be found at CTAN:

http://www.ctan.org/tex-archive/macros/latex/contrib/IEEEtran/bibtex/

as well as within IEEE's site:

http://www.ieee.org/

Note that the packages at IEEE's site do not contain the natbib and
alphanumeric variants (e.g., IEEEtranN.bst, etc.) as these are not used
for IEEE related work. These files can be obtained on CTAN.

For helpful tips, answers to frequently asked questions and other support,
visit the IEEEtran home page at my website:

http://www.michaelshell.org/tex/ieeetran/


Enjoy!

Michael Shell
http://www.michaelshell.org/

*******
Version 1.12 (2007/01/11) changes:

 1. Fixed bug with unwanted comma before "et al." when an entry contained
    more than two author names. Thanks to Pallav Gupta for reporting this.

 2. Fixed bug with anomalous closing quote in tech reports that have a
    type, but without a number or address. Thanks to Mehrdad Mirreza for
    reporting this.

 3. Use braces in \providecommand in begin.bib to better support
    latex2html. TeX style length assignments OK with recent versions
    of latex2html - 1.71 (2002/2/1) or later is strongly recommended.
    Use of the language field still causes trouble with latex2html.
    Thanks to Federico Beffa for reporting this.

 4. Added IEEEtran.bst ID and version comment string to .bbl output.

 5. Provide a \BIBdecl hook that allows the user to execute commands
    just prior to the first entry.

 6. Use default urlstyle (is using url.sty) of "same" rather than rm to
    better work with a wider variety of bibliography styles.

 7. Changed month abbreviations from Sept., July and June to Sep., Jul.,
    and Jun., respectively, as IEEE now does. Thanks to Moritz Borgmann
    for reporting this.

 8. Control entry types should not be considered when calculating longest
    label width.

 9. Added alias www for electronic/online.

10. Updated full and abbreviated journal name string definitions in
    IEEEfull.bib and IEEEabrv.bib.

11. New IEEEtranSA.bst, IEEEtranN.bst, and IEEEtranSN.bst variants for
    alphanumeric citation tags and natbib compatibility.


********************************** Files **********************************

README                 - This file.

IEEEtran_bst_HOWTO.pdf - The user manual.

IEEEtran.bst           - The standard IEEEtran BibTeX style file. For use
                         with IEEE work.

IEEEtranS.bst          - A version of IEEEtran.bst that sorts the entries.
                         Some IEEE conferences/publications may use/allow
                         sorted bibliographies.

IEEEexample.bib        - An example BibTeX database that contains the
                         references shown in the user manual.

IEEEabrv.bib           - String definitions for the abbreviated names of
                         IEEE journals. (For use with IEEE work.)
                         
IEEEfull.bib           - String definitions for the full names of IEEE
                         journals. (Do not use for IEEE work.)


Carried on CTAN only, for non-IEEE related work:

IEEEtranSA.bst         - Like IEEEtranS.bst, but with alphanumeric citation
                         tags like alpha.bst. Not for normal IEEE use.

EEEtranN.bst          - Like IEEEtran.bst, but based on plainnat.bst and
                         is compatible with Patrick W. Daly's natbib
                         package. Not for normal IEEE use.

IEEEtranSN.bst         - Sorting version of IEEEtranN.bst. Not for normal
                         IEEE use

***************************************************************************
Legal Notice:
This code is offered as-is without any warranty either expressed or
implied; without even the implied warranty of MERCHANTABILITY or
FITNESS FOR A PARTICULAR PURPOSE! 
User assumes all risk.
In no event shall IEEE or any contributor to this code be liable for
any damages or losses, including, but not limited to, incidental,
consequential, or any other damages, resulting from the use or misuse
of any information contained here.

All comments are the opinions of their respective authors and are not
necessarily endorsed by the IEEE.

This work is distributed under the LaTeX Project Public License (LPPL)
( http://www.latex-project.org/ ) version 1.3, and may be freely used,
distributed and modified. A copy of the LPPL, version 1.3, is included
in the base LaTeX documentation of all distributions of LaTeX released
2003/12/01 or later.
Retain all contribution notices and credits.
** Modified files should be clearly indicated as such, including  **
** renaming them and changing author support contact information. **

File list of work: IEEEtran_bst_HOWTO.pdf, IEEEtran.bst, IEEEtranS.bst,
                   IEEEtranSA.bst, IEEEtranN.bst, IEEEtranSN.bst,
                   IEEEexample.bib, IEEEabrv.bib, IEEEfull.bib
                   
***************************************************************************


==> mainbody/2.related.tex <==
\section{Related Work}
\label{sec:related}

\textbf{Human Motion Prediction.}
HMP has undergone extensive exploration through both traditional machine learning and modern deep learning methodologies. Traditional approaches rely on handcrafted features and state prediction techniques such as linear dynamic systems~\cite{pavlovic2000learning}, Restricted Boltzmann Machines~\cite{taylor2006modeling}, hidden Markov models~\cite{lehrmann2014efficient}, and Gaussian process latent variable models~\cite{wang2005gaussian}. Despite their utility, these methods encounter challenges in capturing intricate dependencies and temporal dynamics, resulting in constrained prediction accuracy and robustness.
Recently, Convolutional Neural Networks~\cite{butepage2017deep,li2018convolutional,cui2021efficient}, Recurrent Neural Networks~\cite{fragkiadaki2015recurrent,gui2018few,corona2020context}, Long Short-Term Memory~\cite{lee2021video,yuan2019ego}, Transformer Networks~\cite{cai2020learning,aksan2021spatio}, Generative Adversarial Networks ~\cite{gui2018adversarial,hernandez2019human,kundu2019bihmp}, and Graph Convolution Networks~\cite{li2020dynamic,dang2021msr,li2022skeleton,wang2023spatio} have demonstrated promising results in learning motion representations, consequently enhancing the precision and reliability of prediction. Diverging from the previous methods delving into the design of a new network architecture or feature extraction techniques, our focus lies in effectively improving the ability of mapping functions to correlate past and future behaviors. This endeavor yields improvements in the precision of motion prediction.

\textbf{Auxiliary Reconstruction Task.} 
The conflation of reconstruction and prediction in HMP essentially introduces a self-supervised task into the model's learning process.
This auxiliary task can be viewed as an augmentation, leveraging the core concept of utilizing extracted motion representations to reconstruct input information. This process enhances the model's proficiency in learning motion representation.
Auxiliary learning has been used in various tasks such as semantic segmentation~\cite{xu2021leveraging}, image and video captioning~\cite{hosseinzadeh2021image,gao2021hierarchical}, and auto-evaluation~\cite{deng2021does}. The objectives of these auxiliary tasks closely align with the primary prediction task, demanding the network to capture inherent motion patterns effectively. Although the reconstruction has been extensively applied in HMP, refining the utilization of this auxiliary learning task needs more attention.

==> mainbody/rebuttal.tex <==
\newpage

%Experimental Validation

%3DPW实验数据集
\begin{table}[!t]%\scriptsize%\tiny
\renewcommand{\thetable}{1}
\centering
\setlength{\tabcolsep}{3pt} % 1.6
\caption{The average prediction MPJPEs across the test set of 3DPW at various prediction time steps.}
\label{tab:3dpw}
\begin{tabular}{lccccccccccc}
\toprule
Method & 100ms & 200ms & 400ms & 600ms & 800ms & 1K ms & Average\\ \hline 
% Traj-GCN  & 19.91 &40.12  &73.74  &93.19  &104.38  &111.72 \\
% Traj-GCN-T&  
% \\ \hline
SPGSN     & 19.71 &40.35 &74.85 &94.62 &105.30 &112.04 &74.48\\
SPGSN-T &  \textcolor{red}{18.71} &\textcolor{red}{38.55} &\textcolor{red}{72.56} &\textcolor{red}{92.51} &\textcolor{red}{104.26} &\textcolor{red}{111.55} &\textcolor{red}{73.02}\\ \bottomrule
STBMPT    & 19.99 	&41.19 &76.48  	&97.41 	&110.45	&119.79 & 77.55\\
STBMPT-T  &  \textcolor{red}{13.85} &\textcolor{red}{31.07} &\textcolor{red}{66.64} &\textcolor{red}{90.63} &\textcolor{red}{106.23}&\textcolor{red}{117.09} &\textcolor{red}{70.92}\\ %\hline
% STBMPS    & 16.39 	&36.33	&75.50	&101.70 &118.18 &128.85 &79.49 \\
% STBMPS-T  & 16.68 &36.42 &73.58 &97.27  &112.99 &123.41 
%  &\textcolor{red}{76.73}\\ 
\bottomrule
\end{tabular}
\end{table}

%计算代价对比
\begin{table}[!t]%\scriptsize%\footnotesize
\renewcommand{\thetable}{2}
\setlength{\tabcolsep}{4.5pt} 
\centering
\caption{Time and model size comparisons. The average MPJPE at 80ms, 160ms, 320ms, and 400ms is also reported.}
\label{tab:Time and mode size comparisons}
\begin{tabular}{lcccccccccc}
\toprule
 Method & Train(Per batch) & Test(Per batch) & Model Size &MPJPE \\ \hline 
 Traj-GCN  & 52ms & 27ms &2.56M & 37.31 \\
 Traj-GCN-T& 55ms & 29ms & 2.58M & \textcolor{red}{36.26} \\ \hline 
 SPGSN     & 144ms & 68ms & 5.67M  & 34.88 \\  
 SPGSN-T   & 152ms & 71ms & 5.69M  & \textcolor{red}{34.32} \\ \hline %
 STBMPT    & 15ms & 11ms & 3.43M & 36.34\\ 
 STBMPT-T  & 21ms & 13ms & 3.51M  & \textcolor{red}{35.79} \\ \hline
 STBMPS    & 15ms & 10ms & 3.92M & 34.29\\ 
 STBMPS-T  & 19ms & 14ms & 3.94M  & \textcolor{red}{34.04} \\ 
 \bottomrule
\end{tabular}
\end{table}


We appreciate all reviewers for their efforts and time. Your valuable comments greatly improved the quality of our paper. Next, we will reply to each reviewer separately.

\textcolor{blue}{\textbf{Response to the Reviewer $\#1$.}} 
Thank you for your recognition of our work. 
To further validate the effectiveness of our method, we conducted the following additional experiments:
1) \textbf{3DPW}: We evaluated our approach on the 3DPW dataset, which includes over 51,000 frames of challenging indoor and outdoor activities. The official organizers have defined data splits for training, validation, and testing, along with evaluation protocols. The average MPJPEs across all the test samples at different prediction steps are presented in~\tablename{~\ref{tab:3dpw}}. The predictive models with our method consistently outperform the original models.
2) \textbf{Time and Model Size Comparisons}: 
In~\tablename~\ref{tab:Time and mode size comparisons}, we evaluate the computational efficiency of our method in terms of prediction time and model size and present the prediction results for short-term motion prediction in H3.6M. The models with our method consistently exhibit superior performance with slightly increased computational costs. 
3) \textbf{Transformer-Based Model}: We integrated our method into the Transformer-based method AuxFormer (Auxiliary Tasks Benefit 3D Skeleton-based Human Motion Prediction). 
To evaluate the effectiveness of the proposed method, we
carry out five experiments for each combination between
the original and proposed method.
The results, presented in~\tablename{~\ref{tab:h3.6m-aux}}, demonstrate consistent improvements in predictive performance, highlighting the broad applicability of our approach.
4) \textbf{Time Series Prediction Task}: 
We experimented with time series prediction (~\tablename~\ref{tab:tsp}), where our method consistently showed enhanced predictive performance. These findings indicate the potential of our approach in other prediction tasks.

% Taken together, our proposed method exhibits promising results in enhancing both short-term and long-term motion prediction across diverse model architectures and tasks.

%在simPLe和Auxformer增加了实验
\begin{table}[h]%\footnotesize|tiny
\renewcommand{\thetable}{3}
\centering
\setlength{\tabcolsep}{3pt} % 设置列间距为3.5pt 5
\caption{Average prediction MPJPEs on H3.6M. 
}
\label{tab:h3.6m-aux}
\begin{tabular}{lccccccc}
\toprule
 \multirow{1}{*}{Mothod}  & 80ms & 160ms & 320ms & 400ms & 560ms & 1000ms &Average\\ \hline
 % % siMLPe  & 9.64 & 21.83 & 46.53 & 57.51 & 76.05 & 109.68\\ 9.65 	21.85 	46.58 	57.55 	76.20 	109.87 
 % siMLPe  & 9.70 &22.09 &47.29 &58.53 &76.89 &110.26 &54.13\\
 % siMLPe-D  & \textbf{9.68} &\textbf{21.99} &\textbf{46.97} &\textbf{57.99} &\textbf{76.43} &\textbf{110.05} &\textbf{53.85}  \\ \hline
 AuxFormer & 10.00 &21.91 &46.92 &58.34 &78.98 &111.51 & 54.61\\
 AuxFormer-T & \textcolor{red}{9.21} &\textcolor{red}{21.01} &\textcolor{red}{45.77} &\textcolor{red}{57.15} & \textcolor{red}{77.06} &\textcolor{red}{109.60} &\textcolor{red}{53.37}\\
\bottomrule
\end{tabular}
\end{table}

%移植到时间序列预测任务上的实验结果
\begin{table}[h]%\footnotesize|tiny
\renewcommand{\thetable}{4}
\centering
\setlength{\tabcolsep}{8pt} % 设置列间距为3.5pt 5
\caption{Results for the long-term forecasting task under different prediction lengths following the setting of iTransformer in the Traffic dataset.}
\label{tab:tsp}
\begin{tabular}{lcccccc}
\toprule
\multirow{2}{*}{Length} & \multicolumn{2}{l}{iTransformer} & \multicolumn{2}{l}{iTransformer-T} \\ \cmidrule(r){2-3}\cmidrule(){4-5}
 & MSE & MAE & MSE & MAE \\ \hline
16  & 0.395 & 0.268 & \textcolor{red}{0.392} & 0.268\\
192 & 0.417 & \textcolor{red}{0.276} & \textcolor{red}{0.413} & 0.277\\
336 & 0.424 & 0.283 & 0.424 & 0.283\\
720 & 0.467 & 0.302 & \textcolor{red}{0.458} & \textcolor{red}{0.300}\\ \hline
Avg.& 0.428 &0.282 &\textcolor{red}{0.422} &0.282\\
\bottomrule
\end{tabular}
\end{table}

\textbf{\textcolor{magenta}{Response to the Reviewer $\#2$.}} 
We sincerely appreciate your recognition of our work. 
To further validate the effectiveness and robustness of our method, we conducted experiments about 3DPW, time series prediction task, and comparisons of time and model size, as shown in ~\tablename~\ref{tab:3dpw} to ~\tablename~\ref{tab:tsp}. The results demonstrate that our proposed method exhibits promising results in enhancing both short-term and long-term motion prediction across diverse model architectures and tasks.

\textbf{\textcolor{cyan}{Response to the Reviewer $\#3$.}}
%While there is improvement, it is marginal.The key contribution of the paper is in decoupling learning of historical and future motion. But the performance improvement is not significant.
%提升性能不显著
Thank you for your recognition of our work. 
While the improvements may seem marginal in absolute values, they are consistent across various baselines and prediction horizons, highlights the robustness and generalizability of our approach. 
Small gains in HMP are often challenging to achieve and can provide significant benefits, such as improved stability and reduced error accumulation in long-term predictions. Besides, our method enhances model performance without substantial increases in model complexity or computational costs, making it a valuable addition to existing frameworks. Besides, we conducted experiments about 3DPW, time series prediction task, and comparisons of time and model size to further validate the effectiveness and robustness of our method. Please refer to our response to Reviewer $\#1$ for more details.

\textbf{\textcolor{violet}{Response to the Reviewer $\#4$.}}
%The paper follows a common approach of enhancing prediction task through auxiliary tasks: reconstruction. This strategy has been used in various fields, so the core technique, using an auxiliary task for better feature learning, is not novel, even though its application to HMP has unique elements.
%However, the novelty of the approach is somewhat limited, as it relies on the established strategy of using auxiliary tasks.
Thank you for your recognition of our work. 
As illustrated in Fig.1 and Fig.2, there exists a significant difference in the difficulty between reconstructing historical motion and predicting future poses. Existing methods often treat both tasks equally under a shared decoder, neglecting the potential bidirectional correlation between future and historical information, thus hindering the model's effectiveness.
In response to these observations, we propose to decouple the prediction and reconstruction tasks to alleviate the constraints imposed by the reconstruction auxiliary task on the primary prediction task. Besides, we propose an inverse processing to leverage and encourage the potential bidirectional correlation. To the best of our knowledge, our paper is the first to explore the decoupling of tasks and the potential bidirectional correlation in human motion prediction. Moreover, we conducted experiments about 3DPW, time series prediction tasks, and comparisons of time and model size to further validate the effectiveness and robustness of our method, please refer to the response to Reviewer $\#1$ for more details.
% Extensive experimental results validate the effectiveness of our method.
